Advancing Frontiers of Path Integral Theory for Stochastic Optimal Control

Stochastic Optimal Control (SOC) problems arise in systems influenced by uncertainty, such as autonomous robots or financial models. Traditional methods like dynamic programming are often intractable for high-dimensional, nonlinear systems due to the curse of dimensionality. This dissertation explores the path integral control framework as a scalable, sampling-based alternative. By reformulating SOC problems as expectations over stochastic trajectories, it enables efficient policy synthesis via Monte Carlo sampling and supports real-time implementation through GPU parallelization. We apply this framework to six classes of SOC problems: Chance-Constrained SOC, Stochastic Differential Games, Deceptive Control, Task Hierarchical Control, Risk Mitigation of Stealthy Attacks, and Discrete-Time LQR. A sample complexity analysis for the discrete-time case is also provided. These contributions establish a foundation for simulator-driven autonomy in complex, uncertain environments.

==> figs/deception/log_like_cleaned.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\begin{tikzpicture}
\begin{axis}[%
width=2.8in,
height=1.3in,
at={(0in,0in)},
scale only axis,
xmin=0,
xmax=49,
xlabel style={font=\color{white!15!black}},
xlabel={$t$},
ymin=0,
ymax=80,
ylabel style={font=\color{white!15!black}},
ylabel={Log Likelihood Ratio},
axis background/.style={fill=white},
axis x line*=bottom,
axis y line*=left,
xmajorgrids,
ymajorgrids,
legend style={at={(0,0.55)}, anchor=south west, legend cell align=left, align=left, draw=white!15!black}
]
\addplot[area legend, draw=mypurple, fill=mypurple, fill opacity=0.2, forget plot]
table[row sep=crcr] {%
x	y\\
0   0\\
1	3.5523113582886\\
2	7.20496656647935\\
3	10.576139716813\\
4	14.078202679469\\
5	17.5845574074926\\
6	21.1540299643263\\
7	24.6275939214113\\
8	27.9759698955718\\
9	31.2314439614172\\
10	34.6790230395343\\
11	37.8732031172596\\
12	40.7277604950645\\
13	43.5156816762281\\
14	46.2314587265719\\
15	48.5445775952152\\
16	50.5518842586048\\
17	52.230399733868\\
18	53.9192396382854\\
19	55.377708276403\\
20	56.5820476218107\\
21	57.6891517464069\\
22	58.6699540934099\\
23	59.4310609309446\\
24	60.2608522721388\\
25	61.0454106975198\\
26	61.8051765409449\\
27	62.547683061639\\
28	63.2546173863369\\
29	63.7959277784103\\
30	64.3227853817026\\
31	64.7796699928003\\
32	65.2539091454383\\
33	65.6790346633522\\
34	66.0930666011181\\
35	66.3984734411413\\
36	66.6429747222277\\
37	66.8482309623852\\
38	66.9507296944311\\
39	67.0141720407168\\
40	67.1926642307962\\
41	67.269319004698\\
42	67.2504170922385\\
43	67.253134267294\\
44	67.253134267294\\
45	67.253134267294\\
46	67.253134267294\\
47	67.253134267294\\
48	67.253134267294\\
49	67.253134267294\\
49	46.808764862585\\
48	46.808764862585\\
47	46.808764862585\\
46	46.808764862585\\
45	46.808764862585\\
44	46.808764862585\\
43	46.808764862585\\
42	46.807353864224\\
41	46.8157682758702\\
40	46.8192830974176\\
39	46.8027805402073\\
38	46.7866490193912\\
37	46.784399554916\\
36	46.6908552038373\\
35	46.4966377215893\\
34	46.3056958135099\\
33	46.0036919080726\\
32	45.7242018791232\\
31	45.3402475008855\\
30	45.021197733381\\
29	44.5696221245557\\
28	44.0406360095486\\
27	43.4604226686005\\
26	42.8775133011866\\
25	42.1949060301525\\
24	41.3639764156124\\
23	40.5471359062307\\
22	39.6789213690612\\
21	38.7740358425081\\
20	37.8476024186979\\
19	36.9656979340807\\
18	35.969610368931\\
17	35.0473988661163\\
16	33.9377739289592\\
15	32.6973018048621\\
14	31.3585661900023\\
13	30.0116558033631\\
12	28.5719782109428\\
11	27.0079519215159\\
10	25.3291833683109\\
9	23.5049140307571\\
8	21.674751623475\\
7	19.4069333634583\\
6	17.0918754207325\\
5	14.5506767292436\\
4	11.9822749725825\\
3	9.06336326434564\\
2	5.96926520751336\\
1	3.14825720816768\\
0   0\\
}--cycle;
\addplot [color=mypurple, line width=2.0pt]
table[row sep=crcr]{%
0   0\\
1	3.35028428322814\\
2	6.58711588699636\\
3	9.81975149057933\\
4	13.0302388260258\\
5	16.0676170683681\\
6	19.1229526925294\\
7	22.0172636424348\\
8	24.8253607595234\\
9	27.3681789960872\\
10	30.0041032039226\\
11	32.4405775193877\\
12	34.6498693530036\\
13	36.7636687397956\\
14	38.7950124582871\\
15	40.6209397000387\\
16	42.244829093782\\
17	43.6388992999922\\
18	44.9444250036082\\
19	46.1717031052418\\
20	47.2148250202543\\
21	48.2315937944575\\
22	49.1744377312355\\
23	49.9890984185876\\
24	50.8124143438756\\
25	51.6201583638362\\
26	52.3413449210657\\
27	53.0040528651198\\
28	53.6476266979427\\
29	54.182774951483\\
30	54.6719915575418\\
31	55.0599587468429\\
32	55.4890555122807\\
33	55.8413632857124\\
34	56.199381207314\\
35	56.4475555813653\\
36	56.6669149630325\\
37	56.8163152586506\\
38	56.8686893569111\\
39	56.9084762904621\\
40	57.0059736641069\\
41	57.0425436402841\\
42	57.0288854782312\\
43	57.0309495649395\\
44	57.0309495649395\\
45	57.0309495649395\\
46	57.0309495649395\\
47	57.0309495649395\\
48	57.0309495649395\\
49	57.0309495649395\\
};
\addlegendentry{$\lambda\text{=0.5}$}
\addplot[area legend, draw=myblue, fill=myblue, fill opacity=0.2, forget plot]
table[row sep=crcr] {%
x	y\\
0   0\\
1	3.68974822977369\\
2	6.7972644520095\\
3	9.38543211259055\\
4	11.9043583149055\\
5	14.5326506621581\\
6	17.1809740364021\\
7	20.0358275161012\\
8	22.5650544425348\\
9	25.1280396806548\\
10	27.3294487177382\\
11	29.7279388753054\\
12	31.9432827057434\\
13	34.2645694267736\\
14	36.3078980913001\\
15	38.0446298310036\\
16	39.5593689387384\\
17	41.1592653399141\\
18	42.3288754370975\\
19	43.3829401871138\\
20	44.3447628218307\\
21	45.3613528979312\\
22	46.2862115848541\\
23	46.8839824972519\\
24	47.7246576008141\\
25	48.3687929830624\\
26	48.9804144308449\\
27	49.4558511383643\\
28	50.0223862875406\\
29	50.3382515573767\\
30	50.8142049430412\\
31	51.1068728704239\\
32	51.4129884142995\\
33	51.5700784332399\\
34	51.7371304673028\\
35	51.9139593898299\\
36	52.0074718858427\\
37	52.0722828449114\\
38	52.1108174479888\\
39	52.1322563317164\\
40	52.1681364037743\\
41	52.1742507740774\\
42	52.1693294299892\\
43	52.1688977616659\\
44	52.1688977616659\\
45	52.1688977616659\\
46	52.1688977616659\\
47	52.1688977616659\\
48	52.1688977616659\\
49	52.1688977616659\\
49	34.1693023540236\\
48	34.1693023540236\\
47	34.1693023540236\\
46	34.1693023540236\\
45	34.1693023540236\\
44	34.1693023540236\\
43	34.1693023540236\\
42	34.1694262662741\\
41	34.1777508776545\\
40	34.1711861017135\\
39	34.1594825975109\\
38	34.104768099393\\
37	34.0577686592914\\
36	34.0185384337867\\
35	33.9228368776827\\
34	33.8234193774794\\
33	33.7721258307008\\
32	33.5465487161976\\
31	33.3260205340514\\
30	32.9818512458462\\
29	32.7974032764656\\
28	32.682106453654\\
27	32.3522702467809\\
26	32.1529965598892\\
25	31.6478836321751\\
24	31.4670295913361\\
23	30.8610155096005\\
22	30.2897447430032\\
21	29.6190511505558\\
20	28.9031796838664\\
19	28.2297197118996\\
18	27.5455623109637\\
17	26.4946527634377\\
16	25.4298047064668\\
15	24.3817083863905\\
14	23.0887020693811\\
13	21.8919203399562\\
12	20.5822375315288\\
11	19.4129075766331\\
10	17.9734560531882\\
9	16.4498805037412\\
8	14.8371921723408\\
7	12.9252701702739\\
6	11.3199043335402\\
5	9.30252921945164\\
4	7.37122402582956\\
3	5.44296746690072\\
2	3.11537395011982\\
1	1.31411661975003\\
}--cycle;
\addplot [color=myblue, line width=2.0pt]
table[row sep=crcr]{%
0   0\\
1	2.50193242476186\\
2	4.95631920106466\\
3	7.41419978974564\\
4	9.63779117036751\\
5	11.9175899408049\\
6	14.2504391849712\\
7	16.4805488431875\\
8	18.7011233074378\\
9	20.788960092198\\
10	22.6514523854632\\
11	24.5704232259693\\
12	26.2627601186361\\
13	28.0782448833649\\
14	29.6983000803406\\
15	31.213169108697\\
16	32.4945868226026\\
17	33.8269590516759\\
18	34.9372188740306\\
19	35.8063299495067\\
20	36.6239712528485\\
21	37.4902020242435\\
22	38.2879781639286\\
23	38.8724990034262\\
24	39.5958435960751\\
25	40.0083383076187\\
26	40.5667054953671\\
27	40.9040606925726\\
28	41.3522463705973\\
29	41.5678274169211\\
30	41.8980280944437\\
31	42.2164467022377\\
32	42.4797685652485\\
33	42.6711021319703\\
34	42.7802749223911\\
35	42.9183981337563\\
36	43.0130051598147\\
37	43.0650257521014\\
38	43.1077927736909\\
39	43.1458694646136\\
40	43.1696612527439\\
41	43.1760008258659\\
42	43.1693778481317\\
43	43.1691000578448\\
44	43.1691000578448\\
45	43.1691000578448\\
46	43.1691000578448\\
47	43.1691000578448\\
48	43.1691000578448\\
49	43.1691000578448\\
};
\addlegendentry{$\lambda\text{=2}$}
\addplot[area legend, draw=mygreen, fill=mygreen, fill opacity=0.2, forget plot]
table[row sep=crcr] {%
x	y\\
0   0\\
1	3.3926275682848\\
2	5.75930091314732\\
3	8.25439879532083\\
4	10.5441311230055\\
5	12.5336364861145\\
6	14.2607761768403\\
7	16.2423824263045\\
8	17.7337115339871\\
9	19.4394845763661\\
10	20.9845373855114\\
11	22.0792138227822\\
12	23.4879634560568\\
13	24.9642819968042\\
14	26.3361326147128\\
15	27.4269453676147\\
16	28.1365253854545\\
17	29.0906690104725\\
18	30.3820751817646\\
19	31.3727550787652\\
20	31.9049114876835\\
21	32.7225960552991\\
22	33.3481134533472\\
23	34.0422140676238\\
24	34.7467869772092\\
25	35.2482174844241\\
26	35.6938403265812\\
27	36.1206325668433\\
28	36.4869511982949\\
29	36.8291777531083\\
30	37.1071004037322\\
31	37.28929793226\\
32	37.3200930429127\\
33	37.4441942319657\\
34	37.540649963159\\
35	37.6089424789959\\
36	37.677048532227\\
37	37.7018796056384\\
38	37.7747948008681\\
39	37.7817978047797\\
40	37.7975382857611\\
41	37.8043532686747\\
42	37.7959305119219\\
43	37.7960903075025\\
44	37.7960907142633\\
45	37.7960907142633\\
46	37.7960907142633\\
47	37.7960907142633\\
48	37.7960907142633\\
49	37.7960907142633\\
49	21.9745743453596\\
48	21.9745743453596\\
47	21.9745743453596\\
46	21.9745743453596\\
45	21.9745743453596\\
44	21.9745743453596\\
43	21.9745742418702\\
42	21.9745335065502\\
41	21.9739095702949\\
40	21.9738813944456\\
39	21.9771528227097\\
38	21.9527938411261\\
37	21.9174058923014\\
36	21.8743667961828\\
35	21.9193103200879\\
34	21.8526092959341\\
33	21.820414350796\\
32	21.7576781414427\\
31	21.6839991401883\\
30	21.5353969313293\\
29	21.3440804351115\\
28	21.3151011990981\\
27	21.2081338899867\\
26	20.952574308894\\
25	20.6315137104683\\
24	20.4320016726946\\
23	20.1398267183692\\
22	19.8188846002473\\
21	19.3552201294087\\
20	18.8488788690491\\
19	18.2098382292539\\
18	17.7042223657973\\
17	17.215667740551\\
16	16.4770131881503\\
15	15.8660054579197\\
14	15.1625275082077\\
13	13.9811277316788\\
12	12.8383705687737\\
11	12.2093786399307\\
10	11.0354175748587\\
9	10.0027812006316\\
8	8.6765059546501\\
7	7.47568116585045\\
6	6.28508924009862\\
5	5.38808050998785\\
4	3.97459329537258\\
3	2.74294018689862\\
2	1.58616770184121\\
1	0.446107440668074\\
0   0\\
}--cycle;
\addplot [color=mygreen, line width=2.0pt]
table[row sep=crcr]{%
0   0\\
1	1.91936750447644\\
2	3.67273430749426\\
3	5.49866949110972\\
4	7.25936220918905\\
5	8.96085849805115\\
6	10.2729327084695\\
7	11.8590317960775\\
8	13.2051087443186\\
9	14.7211328884988\\
10	16.0099774801851\\
11	17.1442962313565\\
12	18.1631670124152\\
13	19.4727048642415\\
14	20.7493300614602\\
15	21.6464754127672\\
16	22.3067692868024\\
17	23.1531683755117\\
18	24.0431487737809\\
19	24.7912966540096\\
20	25.3768951783663\\
21	26.0389080923539\\
22	26.5834990267972\\
23	27.0910203929965\\
24	27.5893943249519\\
25	27.9398655974462\\
26	28.3232073177376\\
27	28.664383228415\\
28	28.9010261986965\\
29	29.0866290941099\\
30	29.3212486675307\\
31	29.4866485362242\\
32	29.5388855921777\\
33	29.6323042913808\\
34	29.6966296295465\\
35	29.7641263995419\\
36	29.7757076642049\\
37	29.8096427489699\\
38	29.8637943209971\\
39	29.8794753137447\\
40	29.8857098401033\\
41	29.8891314194848\\
42	29.885232009236\\
43	29.8853322746864\\
44	29.8853325298114\\
45	29.8853325298114\\
46	29.8853325298114\\
47	29.8853325298114\\
48	29.8853325298114\\
49	29.8853325298114\\
};
\addlegendentry{$\lambda\text{=3}$}
\end{axis}
\end{tikzpicture}%
